A Survey on Honeypot Software and Data Analysis

In this survey, we give an extensive overview on honeypots. This includes not only honeypot software but also methodologies to analyse honeypot data.

==> text/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

write outro

